Graph Signal Processing: Modulation, Convolution, and Sampling

To analyze data supported by arbitrary graphs G, DSP has been extended to Graph Signal Processing (GSP) by redefining traditional DSP concepts like shift, filtering, and Fourier transform among others. This paper revisits modulation, convolution, and sampling of graph signals as appropriate natural extensions of the corresponding DSP concepts. To define these for both the vertex and the graph frequency domains, we associate with generic data graph G and its graph shift A, a graph spectral shift M and a spectral graph Gs. This leads to a spectral GSP theory that parallels in the graph frequency domain the existing GSP theory in the vertex domain. The paper applies this to design and recovery sampling techniques for data supported by arbitrary directed graphs.

==> auxiliar-2.tex <==
	\section{Convolution in GSP}
	\subsection{Convolution in the Vertex Domain}
	From \cite{DSP} and \cite{Freq}, convolution in the vertex domain is defined as a matrix vector multiplication, shown in Equation \eqref{convtime}.
	
	Let the polynomial filter be:
	\begin{equation}\label{PAeq}
	P(A) = p_{N-1}A^{N-1}+p_{N-2}A^{N-2}+\hdots+p_1A+p_0I
	\end{equation}
	
	We consider the Fourier pair:
	\begin{equation}\label{convpairtime}
	P(A) \ x \xrightarrow{\mathcal{F}} \widehat{y} \odot \widehat{x}
	\end{equation}
	where $x$ and $y$ are signals and $P(A)$ is the polynomial of $A$ defined in \eqref{PAeq}. The GFT of the matrix vector product between matrix $P(A)$ and vector x is the pointwise product of signals $\widehat{x}$ and $\widehat{y}$. We relate now the matrix $P(A)$ with the signal $\widehat{y}$.
	
	Using Equation \eqref{Adecompgsp}, we substitute $A$ into Equation \eqref{convtime}. This yields:
	\begin{align*}
	P(A)x &= \textrm{GFT}^{-1}\Big(p_{N-1}\Lambda^{N-1}+p_{N-2}\Lambda^{N-2}\\  &\hspace{1cm}+\hdots+p_1\Lambda+p_0\Big)\textrm{GFT}x \\
	&= \textrm{GFT}^{-1}\Big(p_{N-1}\Lambda^{N-1}+p_{N-2}\Lambda^{N-2}\\
	&\hspace{1cm}+ \hdots+p_1\Lambda+p_0\Big) \widehat{x} \\
	&= \textrm{GFT}^{-1}P(\Lambda) \widehat{x}
	\end{align*}
	
	Taking the GFT of $P(A)x$ yields:
	\begin{equation} \label{result1}
	P(\Lambda)\widehat{x} = \widehat{y} \odot \widehat{x}
	\end{equation}
	Since $\Lambda$ is a diagonal matrix, $P(\Lambda)$ is also diagonal. Thus,
	\begin{equation} \label{systemtime}
	P(\Lambda) = \textrm{diag}(\widehat{y})
	\end{equation}
	
	We also have:
	\begin{equation} \label{Apoly}
	P(A) = \textrm{GFT}^{-1} \ P(\Lambda) \ \textrm{GFT}
	\end{equation}
	Substituting \eqref{systemtime} into \eqref{Apoly} yields:
	\begin{equation} \label{convtimeans}
	P(A) = \textrm{GFT}^{-1} \ \textrm{diag}(\widehat{y}) \ \textrm{GFT}
	\end{equation}
	
	Thus, the pointwise product, $\odot$, of signals $\widehat{x}$ and $\widehat{y}$ in the frequency domain  is the matrix vector product of matrix $\textrm{GFT}^{-1} \ \textrm{diag}(\widehat{y}) \ \textrm{GFT}$ and signal $\widehat{x}$.
	
	\subsection{Convolution in the Spectral Domain}
	Using equation \eqref{Mgeqn}, we consider convolution in the spectral domain in GSP.
	Similar to convolution in the vertex domain, we consider the Fourier pair:
	\begin{equation}\label{convpair}
	y \odot x \xrightarrow{\mathcal{F}} P(M) \ \widehat{x}
	\end{equation}
	where $x$ and $y$ are signals and $P(M)$ is a polynomial of the graph shift in frequency, $M$. The graph Fourier transform of the pointwise product of signals $x$ and $y$ is a matrix vector product between matrix $P(M)$ and vector $x$.
	The matrix $P(M)$ is related to the signal $y$ being multiplied in the vertex domain.
	
	Assume there are $N$ nodes in the arbitrary graph. Let $P(M)$ be a polynomial of degree $N-1$ of $M$. $P(M)$ has the form:
	\begin{equation}\label{PMeq}
	P(M) = p_{N-1}M^{N-1}+p_{N-2}M^{N-2}+\hdots+p_1M+p_0I
	\end{equation}
	
	Using equations \eqref{Mgeqn}, \eqref{convpair} and \eqref{PMeq},
	\begin{align*}
	P(M) \widehat{x} &= \textrm{GFT} \ \Big(p_{N-1}\Lambda^{*^{N-1}}+p_{N-2}\Lambda^{*^{N-2}}\\
	&\hspace{1cm}+\hdots+p_1\Lambda^*+p_0\Big) \ \textrm{GFT}^{-1} \widehat{x} \\
	&= \textrm{GFT} \ \Big(p_{N-1}\Lambda^{*^{N-1}}+p_{N-2}\Lambda^{*^{N-2}}\\
	&\hspace{1cm}+\hdots+p_1\Lambda^*+p_0\Big) x\\
	&= \textrm{GFT} P(\Lambda^*) x
	\end{align*}
	
	Taking the inverse GFT of $P(M)\widehat{x}$ yields:
	\begin{equation} \label{result2}
	P(\Lambda^*) x = y \odot x
	\end{equation}
	Since $\Lambda^*$ is a diagonal matrix, $P(\Lambda^*)$ is also diagonal. Thus,
	\begin{equation} \label{system}
	P(\Lambda^*) = \textrm{diag}(y)
	\end{equation}
	We also have:
	\begin{equation} \label{Apolyf}
	P(M) = \textrm{GFT} \ P(\Lambda^*) \ \textrm{GFT}^{-1}
	\end{equation}
	Substituting \eqref{system} into Equation \eqref{Apolyf} yields:
	\begin{equation} \label{convfreqans}
	P(M) = \textrm{GFT} \ \textrm{diag}(y) \ \textrm{GFT}^{-1}
	\end{equation}
	Thus, the pointwise product, $\odot$, of two signals, $x$ and $y$, in the vertex domain is the matrix vector product of matrix $\textrm{GFT} \ \textrm{diag}(y) \ \textrm{GFT}^{-1}$ and signal $x$ in the spectral domain.
	
	\subsection{Polynomials of the Shift}
	In the previous two sections, we illustrated two ways
	
	
	
	
	
	
	
	\subsection{Scaling Constants}
	The eigendecomposition of $A$ is subject to scaling constants. The GFT matrix can be scaled by a factor of $k$ and the $\textrm{GFT}^{-1}$ can be scaled by a factor of $\frac{1}{k}$.
	For example, suppose $A$ has eigendecomposition, $A = \textrm{GFT}^{-1} \ \Lambda \ \textrm{GFT}$. Then,
	\begin{equation} \label{alteigen}
	A = k \ \textrm{GFT}^{-1} \ \Lambda \ \textrm{GFT} \ \frac{1}{k}
	\end{equation}
	where $k \in \mathbb{R}$, $k \neq 0$ is also a valid eigendecomposition of $A$. However, the GFT and $\textrm{GFT}^{-1}$ have been scaled by constants, producing different numerical results and Fourier pairs. Because of this, we now introduce a generic form of Equation \eqref{convpairtime}:
	\begin{equation}\label{convpairtimegen}
	P(A) \ x \xrightarrow{\mathcal{F}} k\ \left(\widehat{y} \odot \widehat{x}\right)
	\end{equation}
	where $x$ and $y$ are signals, $k \in \mathbb{R}$ is a scalar, and $P(A)$ is the polynomial of $A$.
	Based on Equation \eqref{convpairtimegen}, using a similar argument as in Section A, we can derive the following generic form of Equation \eqref{convtimeans}.
	\begin{align}
	    P(\Lambda)\widehat{x} &= k\left(\widehat{y}\odot\widehat{x}\right) \nonumber\\
	    P(\Lambda) &= k\left(\textrm{diag}(\widehat{y})\right) \nonumber\\
	    P(A) &= k \left( \textrm{GFT}^{-1} \ \textrm{diag}(\widehat{y}) \ \textrm{GFT}\right)  \label{convtimeansgen}
	\end{align}
	
	Similarly, for convolution in the spectral domain, we introduce a generic form of Equation \eqref{convpair}:
	\begin{equation}\label{convpairgen}
	l\left(y \odot x\right) \xrightarrow{\mathcal{F}} P(M) \ \widehat{x}
	\end{equation}
	where $x$ and $y$ are signals, $l\in \mathbb{R}$ is a scalar and $P(M)$ is a polynomial of the graph shift in frequency, $M$. Based on Equation \eqref{convpairgen}, using a similar argument as in Section B, we can derive a generic form of Equation \eqref{convfreqans}.
	\begin{align}
	    P(\Lambda^*)x &= l\left(y \odot x\right) \nonumber\\
	    P(\Lambda^*) &= l\left(\textrm{diag}(y)\right) \nonumber\\
	    P(M) &= l \left( \textrm{GFT} \ \textrm{diag}(y) \ \textrm{GFT}^{-1}\right)  \label{convfreqansgen}
	\end{align}

	This theory is also consistent with DSP by considering matrix $M$ in equation \eqref{Meqn} and the adjacency matrix $A$ of the $N$ node ring graph. We will illustrate this theoretically and by example in the next sections.
	\subsection{DSP Convolution in Time}
	We consider the $N$ node ring graph with adjacency matrix $A$. Let $x$ and $y$ be $N \times 1$ discrete time signals.
	
	In DSP,
	\begin{equation}\label{convform}
	x * y = \sum_{k = 0}^{N-1} y_{n-k}x_{k}
	\end{equation}
	Equation \eqref{convform} can be written as the following matrix vector multiplication:
	\begin{align}
	x * y &= \begin{bmatrix}
	y_0  & y_{N-1} & y_{N-2} & \hdots & y_{2} & y_{1} \\
	y_{1}  & y_{0} & y_{N-1} &  \hdots & y_{3} & y_{2} \\
	y_{2}  & y_{1} & y_{0} &  \hdots & y_{4} & y_{3} \\
	\vdots  & \vdots & \vdots & \ddots & \vdots  & \vdots\\
	y_{N-2}  & y_{N-3} & y_{N-4} &  \hdots & y_{0} & y_{N-1} \\
	y_{N-1}  & y_{N-2} & y_{N-3} &  \hdots & y_{1} & y_{0} \\
	\end{bmatrix} x \label{expandmtx}\\
	&= (y_0I + y_1A + y_2A^2 + \hdots + y_{N-1}A^{N-1})x \nonumber\\
    &= \left(\sum_{i = 0}^{N-1} y_{i}A^{i}\right)x \nonumber\\
	&= P(A)x \nonumber
	\end{align}
	Thus,
	\begin{equation} \label{Apolydsp}
	 P(A) = \sum_{i = 0}^{N-1} y_{i}A^{i}
	\end{equation}
	
    The $N \times N$ unitary DFT is given by:
    \begin{equation} \label{dftmatrix}
    \textrm{DFT} = \frac{1}{\sqrt{N}}\left(e^{-\frac{2\pi j}{N}pq}\right)_{p,q = 0,1,2,\hdots,N-1}
    \end{equation} where $j = \sqrt{-1}$.

    The Fourier pair is:
    \begin{equation}\label{dftfourierpair1}
	P(A) \ x \xrightarrow{\mathcal{F}} \sqrt{N} \ (\widehat{y} \odot \widehat{x})
	\end{equation}

	From Equation \eqref{convtimeansgen} and Equation \eqref{dftfourierpair1}, substituting in the DFT for the GFT and $k = \sqrt{N}$ yields:
	\begin{equation} \label{dftA}
	P(A) = \sqrt{N} \left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \textrm{DFT}\right)
	\end{equation}
	
	\begin{theorem}
	In DSP, the two formulations for $P(A)$ from the DSP convolution definition in Equation \eqref{Apolydsp} and from the GSP theory in Equation \eqref{dftA} are equivalent.
	\end{theorem}
	$P(A) = \sqrt{N} \left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \textrm{DFT}\right) = \sum_{i = 0}^{N-1} y_{i}A^{i}$
	\begin{proof}
	It suffices to show that $\sqrt{N} \left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \textrm{DFT}\right)$ is equal to the matrix of y values in Equation \eqref{expandmtx}.
	
	Let $P = P(A)$. Let $P_i$ denote the $i$th column of $P(A)$.
	\begin{equation} \label{pieq}
	P_i = \sqrt{N}\left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \textrm{DFT}_i\right)
	\end{equation}
    where $\textrm{DFT}_i$ is the $i$th column of the DFT matrix.

    So,
    \begin{equation} \label{dftkmatrix}
    \textrm{DFT}_i = \frac{1}{\sqrt{N}}\left(e^{-\frac{2\pi j}{N}pi}\right)_{p = 0,1,2,\hdots,N-1}
    \end{equation}
    Substituting Equation \eqref{dftkmatrix} into Equation \eqref{pieq}  yields:
    \begin{align*}
	P_i &= \sqrt{N}\left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \textrm{DFT}_i\right)\\
	&= \sqrt{N}\left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \frac{1}{\sqrt{N}}\left(e^{-\frac{2\pi j}{N}pi}\right)_{p = 0,1,2,\hdots,N-1}\right) \\
	&= \textrm{DFT}^{-1} \ \left(\widehat{Y}_p e^{-\frac{2\pi j}{N}pi}\right)_{p = 0,1,2,\hdots,N-1}\\
	&= y_{n-i}
    \end{align*}
    The $i$th column of $P(A)$ is equal to $y_n$ shifted $i$ times. This is precisely the matrix in Equation \eqref{expandmtxfreq}.
    So, $\sqrt{N}\left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{y}) \ \textrm{DFT}\right)$ is equal to the matrix of y values in Equation \eqref{expandmtxfreq}.
    Thus, the two formulations are equivalent.
	\end{proof}
	
	\textit{Example:}
	Let $N = 4$. Let $\widehat{X} = [1,2,3,4]^T$, $\widehat{Y}=[-1,1,2,4]^T$, $\widehat{Y} = \textrm{DFT} \ y=\frac{1}{2}[6,-3+3j,-4,-3-3j]^T$
	
	$A$ is the 4-node ring graph adjacency matrix:
	\begin{equation*}
	A = \begin{bmatrix}
	0  & 0 & 0 & 1 \\
	1  & 0 & 0 & 0 \\
	0 &	 1 & 0 & 0 \\
	0 &	 0 & 1 & 0
	\end{bmatrix}
	\end{equation*}
	
	From Equation \eqref{Apolydsp}, we have
	\begin{align*}
	    P(A) &= -I + A + 2A^2 + 4A^3 \\
	   &=
	\begin{bmatrix}
	-1  & 4 & 2 & 1 \\
	1  & -1 & 4 & 2 \\
	2 &	 1 & -1 & 4 \\
	4 &	 2 & 1 & -1
	\end{bmatrix}
	\end{align*}
	
	From Equation \eqref{dftA} with $k = 2$, we have
	\begin{align*}
	   P(A) &= 2\left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \textrm{DFT}\right)\\
	   &= 2\left(\textrm{DFT}^{-1} \ \textrm{diag}(\frac{1}{2}[6,-3+3j,-4,-3-3j]) \ \textrm{DFT}\right)\\
	   &= \textrm{DFT}^{-1} \ \textrm{diag}([6,-3+3j,-4,-3-3j]) \ \textrm{DFT} \\
	&= \begin{bmatrix}
	-1  & 4 & 2 & 1 \\
	1  & -1 & 4 & 2 \\
	2 &	 1 & -1 & 4 \\
	4 &	 2 & 1 & -1
	\end{bmatrix}
	\end{align*}
	Both formulations yield the matrix of y values detailed in Equation \eqref{expandmtx}.
	
	Thus,
	$x*y = P(A)x = \begin{bmatrix}
	-1  & 4 & 2 & 1 \\
	1  & -1 & 4 & 2 \\
	2 &	 1 & -1 & 4 \\
	4 &	 2 & 1 & -1
	\end{bmatrix} x = \begin{bmatrix}
	-1  & 4 & 2 & 1 \\
	1  & -1 & 4 & 2 \\
	2 &	 1 & -1 & 4 \\
	4 &	 2 & 1 & -1
	\end{bmatrix} [1,2,3,4]^T = [17, 19, 17, 7]^T$
	
	\subsection{DSP Convolution in Frequency}
	We consider the $N$ node ring graph with adjacency matrix $A$. Let $x$ and $y$ be $N \times 1$ discrete time signals. $\widehat{X} = \textrm{DFT}\ x$, $\widehat{Y} = \textrm{DFT}\ y$. From Theorem \ref{AMequal}, we know that the frequency shift, $M = A$.
	
	In DSP,
	\begin{equation}\label{convformfreq}
	\widehat{X} * \widehat{Y} = \sum_{k = 0}^{N-1} {\widehat{Y}_{n-k}\widehat{X}_{k}}
	\end{equation}
	Equation \eqref{convformfreq} can be written as the following matrix vector multiplication:
	\begin{align}
	\widehat{X} * \widehat{Y} &= \begin{bmatrix}
	\widehat{Y}_0  & \widehat{Y}_{N-1} & \widehat{Y}_{N-2} & \hdots & \widehat{Y}_{2} & \widehat{Y}_{1} \\
	\widehat{Y}_{1}  & \widehat{Y}_{0} & \widehat{Y}_{N-1} &  \hdots & \widehat{Y}_{3} & \widehat{Y}_{2} \\
	\widehat{Y}_{2}  & \widehat{Y}_{1} & \widehat{Y}_{0} &  \hdots & \widehat{Y}_{4} & \widehat{Y}_{3} \\
	\vdots  & \vdots & \vdots & \ddots & \vdots  & \vdots\\
	\widehat{Y}_{N-2}  & \widehat{Y}_{N-3} & \widehat{Y}_{N-4} &  \hdots & \widehat{Y}_{0} & \widehat{Y}_{N-1} \\
	\widehat{Y}_{N-1}  & \widehat{Y}_{N-2} & \widehat{Y}_{N-3} &  \hdots & \widehat{Y}_{1} & \widehat{Y}_{0} \\
	\end{bmatrix} \widehat{X} \label{expandmtxfreq}\\
	&= (\widehat{Y}_0I + \widehat{Y}_1M + \widehat{Y}_2M^2 + \hdots + \widehat{Y}_{N-1}M^{N-1})x \nonumber \\
    &= \left(\sum_{i = 0}^{N-1} \widehat{Y}_{i}M^{i}\right)x \nonumber\\
	&= P(M)x \nonumber
	\end{align}
	Thus,
	\begin{equation} \label{Mpolydsp}
	 P(M) = \sum_{i = 0}^{N-1} \widehat{Y}_{i}M^{i}
	\end{equation}
    The $N \times N$ unitary $\textrm{DFT}^{-1}$ is given by:
    \begin{equation} \label{dftmatrixinv}
     \textrm{DFT}^{-1} = \frac{1}{\sqrt{N}}\left(e^{\frac{2\pi j}{N}pq}\right)_{p,q = 0,1,2,\hdots,N-1}
    \end{equation} where $j = \sqrt{-1}$.
    The Fourier pair is:
    \begin{equation}\label{dftfourierpair2}
	\sqrt{N} (\widehat{y} \odot \widehat{x}) \xrightarrow{\mathcal{F}} P(M) \ x
	\end{equation}
	From Equation \eqref{convfreqansgen}, substituting in the DFT for the GFT yields:
	\begin{equation} \label{dftM}
	P(M) = \sqrt{N}\left(\textrm{DFT}\ \textrm{diag}(y) \ \textrm{DFT}^{-1}\right)
	\end{equation}
	
	\begin{theorem}
	In DSP, the two formulations for $P(M)$ from the DSP convolution definition in Equation \eqref{Mpolydsp} and from the GSP theory in Equation \eqref{dftM} are equivalent.
	
    $P(M) = \sqrt{N}\left(\textrm{DFT} \ \textrm{diag}(y) \ \textrm{DFT}^{-1}\right) = \sum_{i = 0}^{N-1} \widehat{Y}_{i}M^{i}$
	\end{theorem}
	
	\begin{proof}
	It suffices to show that $\sqrt{N}\left(\textrm{DFT}\ \textrm{diag}(y) \ \textrm{DFT}^{-1}\right)$ is equal to the matrix of $\widehat{Y}$ values in Equation \eqref{expandmtxfreq}.
	
	Let $P = P(M)$. Let $P_i$ denote the $i$th column of $P(M)$.
	\begin{equation} \label{pieqfreq}
	P_i = \sqrt{N}\left(\textrm{DFT} \ \textrm{diag}(y) \ \textrm{DFT}^{-1}_i\right)
	\end{equation}
    where $\textrm{DFT}^{-1}_i$ is the $i$th column of the $\textrm{DFT}^{-1}$ matrix.



    So,
    \begin{equation} \label{dftkmatrixinv}
    \textrm{DFT}_i = \frac{1}{\sqrt{N}}\left(e^{\frac{2\pi j}{N}pi}\right)_{p = 0,1,2,\hdots,N-1}
    \end{equation}
    Substituting Equation \eqref{dftkmatrixinv} into Equation \eqref{pieqfreq}  yields:
    \begin{align*}
	P_i &= \sqrt{N}\left(\textrm{DFT} \ \textrm{diag}(y) \ \textrm{DFT}^{-1}_i\right)\\
	&= \sqrt{N}\left(\textrm{DFT} \ \textrm{diag}(y) \ \frac{1}{\sqrt{N}}\left(e^{\frac{2\pi j}{N}pi}\right)_{p = 0,1,2,\hdots,N-1}\right) \\
	&= \textrm{DFT} \ \left(y_p e^{-\frac{2\pi j}{N}pi}\right)_{p = 0,1,2,\hdots,N-1} \\
	&= \widehat{Y}_{n-i}
    \end{align*}
    The $i$th column of $P(M)$ is equal to $\widehat{Y}_{n}$ shifted i times. This is precisely the matrix in Equation \eqref{expandmtxfreq}.
    So, $\sqrt{N}\left(\textrm{DFT} \ \textrm{diag}(y) \ \textrm{DFT}^{-1}\right)$ is equal to the matrix of $\widehat{Y}$ values in Equation \eqref{expandmtxfreq}.
    Thus, the two formulations are equivalent.
	\end{proof}
	
	\textit{Example:}
	Let $N = 4$. Let $\widehat{X} = [1,2,3,4]^T$, $\widehat{Y}=[6,-3+3j,-4,-3-3j]^T$, $y = \textrm{DFT}^{-1} \ \widehat{Y}=\frac{1}{2}[-4, 16, 8, 4]^T$
	
	$A$ is the 4-node ring graph adjacency matrix. Using Theorem \ref{AMequal},
	\begin{equation*}
	M = A = \begin{bmatrix}
	0  & 0 & 0 & 1 \\
	1  & 0 & 0 & 0 \\
	0 &	 1 & 0 & 0 \\
	0 &	 0 & 1 & 0
	\end{bmatrix}
	\end{equation*}
	
	From Equation \eqref{Mpolydsp}, we have
	\begin{align*}
	    P(M) &= 6I + (-3+3j)A + -4A^2 + (-3-3j)A^3 \\
	   &=
	\begin{bmatrix}
	6  & -3+3j & -4 & -3-3j \\
	-3-3j  & 6 & -3+3j & -4 \\
	-4 & -3-3j & 6 & -3+3j \\
	-3+3j &	 -4 & -3-3j & 6
	\end{bmatrix}
	\end{align*}
	
	From Equation \eqref{dftM}, we have
	\begin{align*}
	   P(M) &= 2\left(\textrm{DFT} \ \textrm{diag}(y) \ \textrm{DFT}^{-1}\right)\\
	   &= 2\left(\textrm{DFT} \ \textrm{diag}(\frac{1}{2}[-4, 16, 8, 4]) \ \textrm{DFT}^{-1}\right)\\
	   &= \textrm{DFT} \ \textrm{diag}([-4,16,8,4]) \ \textrm{DFT}^{-1}\\
	&= \begin{bmatrix}
	6  & -3+3j & -4 & -3-3j \\
	-3-3j  & 6 & -3+3j & -4 \\
	-4 & -3-3j & 6 & -3+3j \\
	-3+3j &	 -4 & -3-3j & 6
	\end{bmatrix}
	\end{align*}
	Both formulations yield the matrix of y values detailed in Equation \eqref{expandmtxfreq}.
	
	Thus,
	$\widehat{x}*\widehat{y} = P(M)x = \\
	\begin{bmatrix}
	6  & -3+3j & -4 & -3-3j \\
	-3-3j  & 6 & -3+3j & -4 \\
	-4 & -3-3j & 6 & -3+3j \\
	-3+3j &	 -4 & -3-3j & 6
	\end{bmatrix} \widehat{x} =  \\ \begin{bmatrix}
	6  & -3+3j & -4 & -3-3j \\
	-3-3j  & 6 & -3+3j & -4 \\
	-4 & -3-3j & 6 & -3+3j \\
	-3+3j &	 -4 & -3-3j & 6
	\end{bmatrix} [1,2,3,4]^T \\ = [-24-6j, -16+6j, -4+6j, 4-6j]^T$
	


==> auxiliar.tex <==
	\section{Convolution in GSP} \label{sec:gspconvolution}
We consider now convolution in both the vertex and the graph spectral domains.
%
%
	\subsection{Convolution in the Vertex Domain} \label{subsec:gspconvolutionvertex}
	We start with convolution in the vertex domain of two graph signals: $x$ that is input to a to be determined polynomial filter whose impulse response is the graph signal~$y$. From \cite{Sandryhaila:13} and \cite{Sandryhaila:14}, filtering in the vertex domain is defined by a matrix vector multiplication. For shift invariant filters, the matrix filter is a polynomial filter $P(A)$ in the shift~$A$ as shown in Equation \eqref{convtime}. Let the polynomial filter be:
	\begin{align}\label{PAeq}
	P(A){}& = p_{N-1}A^{N-1}+p_{N-2}A^{N-2}+\hdots+p_1A+p_0I.
	\end{align}
	%
	We consider the graph Fourier pair:
	\begin{align}\label{convpairtime}
	P(A) \ x \xrightarrow{\mathcal{F}} \widehat{y} \odot \widehat{x}
	\end{align}
	where $\widehat{x}$ and $\widehat{y}$ are the $\textrm{GFT}$ of the graph signals~$x$  and~$y$, $\widehat{y}$ is the graph spectral response of the filter $P(A)$,  and $\odot$ is the Hadamard or entry wise product of two vectors.  The GFT of the filtering of~$x$ by the shift invariant filter $P(A)$ is the pointwise product of the signals $\widehat{x}$ and $\widehat{y}$. We relate now the matrix $P(A)$ with the signal $\widehat{y}$.
	
	Using Equation \eqref{Adecompgsp}, we substitute $A$ into Equation \eqref{convtime}. This yields:
	\begin{align*}
	P(A)x &= \textrm{GFT}^{-1}\Big(p_{N-1}\Lambda^{N-1}+p_{N-2}\Lambda^{N-2}\\  &\hspace{1cm}+\hdots+p_1\Lambda+p_0\Big)\textrm{GFT}x \\
	&= \textrm{GFT}^{-1}\Big(p_{N-1}\Lambda^{N-1}+p_{N-2}\Lambda^{N-2}\\
	&\hspace{1cm}+ \hdots+p_1\Lambda+p_0\Big) \widehat{x} \\
	&= \textrm{GFT}^{-1}P(\Lambda) \widehat{x}
	\end{align*}
	
	Taking the GFT of $P(A)x$ yields:
	\begin{align} \label{result1}
	P(\Lambda)\widehat{x} = \widehat{y} \odot \widehat{x}
	\end{align}
	Since $\Lambda$ is a diagonal matrix, $P(\Lambda)$ is also diagonal. Thus,
	\begin{align} \label{systemtime}
	P(\Lambda) = \textrm{diag}(\widehat{y})
	\end{align}
	
	We also have:
	\begin{align} \label{Apoly}
	P(A) = \textrm{GFT}^{-1} \ P(\Lambda) \ \textrm{GFT}
	\end{align}
	Substituting \eqref{systemtime} into \eqref{Apoly} yields:
	\begin{align} \label{convtimeans}
	P(A) = \textrm{GFT}^{-1} \ \textrm{diag}(\widehat{y}) \ \textrm{GFT}
	\end{align}
	
	Thus, the pointwise product, $\odot$, of signals $\widehat{x}$ and $\widehat{y}$ in the frequency domain  is the matrix vector product of matrix $\textrm{GFT}^{-1} \ \textrm{diag}(\widehat{y}) \ \textrm{GFT}$ and signal $\widehat{x}$.
	
	\subsection{Convolution in the Spectral Domain} \label{subsec:gspconvolutionspectral}
	Using equation \eqref{Mgeqn}, we consider convolution in the spectral domain in GSP.
	Similar to convolution in the vertex domain, we consider the Fourier pair:
	\begin{align}\label{convpair}
	y \odot x \xrightarrow{\mathcal{F}} P(M) \ \widehat{x}
	\end{align}
	where $x$ and $y$ are signals and $P(M)$ is a polynomial of the graph shift in frequency, $M$. The graph Fourier transform of the pointwise product of signals $x$ and $y$ is a matrix vector product between matrix $P(M)$ and vector $x$.
	The matrix $P(M)$ is related to the signal $y$ being multiplied in the vertex domain.
	
	Assume there are $N$ nodes in the arbitrary graph. Let $P(M)$ be a polynomial of degree $N-1$ of $M$. $P(M)$ has the form:
	\begin{align}\label{PMeq}
	P(M) = p_{N-1}M^{N-1}+p_{N-2}M^{N-2}+\hdots+p_1M+p_0I
	\end{align}
	
	Using equations \eqref{Mgeqn}, \eqref{convpair} and \eqref{PMeq},
	\begin{align*}
	P(M) \widehat{x} &= \textrm{GFT} \ \Big(p_{N-1}\Lambda^{*^{N-1}}+p_{N-2}\Lambda^{*^{N-2}}\\
	&\hspace{1cm}+\hdots+p_1\Lambda^*+p_0\Big) \ \textrm{GFT}^{-1} \widehat{x} \\
	&= \textrm{GFT} \ \Big(p_{N-1}\Lambda^{*^{N-1}}+p_{N-2}\Lambda^{*^{N-2}}\\
	&\hspace{1cm}+\hdots+p_1\Lambda^*+p_0\Big) x\\
	&= \textrm{GFT} P(\Lambda^*) x
	\end{align*}
	
	Taking the inverse GFT of $P(M)\widehat{x}$ yields:
	\begin{align} \label{result2}
	P(\Lambda^*) x = y \odot x
	\end{align}
	Since $\Lambda^*$ is a diagonal matrix, $P(\Lambda^*)$ is also diagonal. Thus,
	\begin{align} \label{system}
	P(\Lambda^*) = \textrm{diag}(y)
	\end{align}
	We also have:
	\begin{align} \label{Apolyf}
	P(M) = \textrm{GFT} \ P(\Lambda^*) \ \textrm{GFT}^{-1}
	\end{align}
	Substituting \eqref{system} into Equation \eqref{Apolyf} yields:
	\begin{align} \label{convfreqans}
	P(M) = \textrm{GFT} \ \textrm{diag}(y) \ \textrm{GFT}^{-1}
	\end{align}
	Thus, the pointwise product, $\odot$, of two signals, $x$ and $y$, in the vertex domain is the matrix vector product of matrix $\textrm{GFT} \ \textrm{diag}(y) \ \textrm{GFT}^{-1}$ and signal $x$ in the spectral domain.
	
	\subsection{Scaling Constants} \label{subsec:scalingconstants}
	The eigendecomposition of $A$ is subject to scaling constants. The GFT matrix can be scaled by a factor of $k$ and the $\textrm{GFT}^{-1}$ can be scaled by a factor of $\frac{1}{k}$.
	For example, suppose $A$ has eigendecomposition, $A = \textrm{GFT}^{-1} \ \Lambda \ \textrm{GFT}$. Then,
	\begin{align} \label{alteigen}
	A = k \ \textrm{GFT}^{-1} \ \Lambda \ \textrm{GFT} \ \frac{1}{k}
	\end{align}
	where $k \in \mathbb{R}$, $k \neq 0$ is also a valid eigendecomposition of $A$. However, the GFT and $\textrm{GFT}^{-1}$ have been scaled by constants, producing different numerical results and Fourier pairs. Because of this, we now introduce a generic form of Equation \eqref{convpairtime}:
	\begin{align}\label{convpairtimegen}
	P(A) \ x \xrightarrow{\mathcal{F}} k\ \left(\widehat{y} \odot \widehat{x}\right)
	\end{align}
	where $x$ and $y$ are signals, $k \in \mathbb{R}$ is a scalar, and $P(A)$ is the polynomial of $A$.
	Based on Equation \eqref{convpairtimegen}, using a similar argument as in Section A, we can derive the following generic form of Equation \eqref{convtimeans}.
	\begin{align}
	    P(\Lambda)\widehat{x} &= k\left(\widehat{y}\odot\widehat{x}\right) \nonumber\\
	    P(\Lambda) &= k\left(\textrm{diag}(\widehat{y})\right) \nonumber\\
	    P(A) &= k \left( \textrm{GFT}^{-1} \ \textrm{diag}(\widehat{y}) \ \textrm{GFT}\right)  \label{convtimeansgen}
	\end{align}
	
	Similarly, for convolution in the spectral domain, we introduce a generic form of Equation \eqref{convpair}:
	\begin{align}\label{convpairgen}
	l\left(y \odot x\right) \xrightarrow{\mathcal{F}} P(M) \ \widehat{x}
	\end{align}
	where $x$ and $y$ are signals, $l\in \mathbb{R}$ is a scalar and $P(M)$ is a polynomial of the graph shift in frequency, $M$. Based on Equation \eqref{convpairgen}, using a similar argument as in Section B, we can derive a generic form of Equation \eqref{convfreqans}.
	\begin{align}
	    P(\Lambda^*)x &= l\left(y \odot x\right) \nonumber\\
	    P(\Lambda^*) &= l\left(\textrm{diag}(y)\right) \nonumber\\
	    P(M) &= l \left( \textrm{GFT} \ \textrm{diag}(y) \ \textrm{GFT}^{-1}\right)  \label{convfreqansgen}
	\end{align}

	This theory is also consistent with DSP by considering matrix $M$ in equation \eqref{Meqn} and the adjacency matrix $A$ of the $N$ node ring graph. We will illustrate this theoretically and by example in the next sections.
	\subsection{DSP Convolution in Time} \label{subsec:dsptimeconvolution}
	We consider the $N$ node ring graph with adjacency matrix $A$. Let $x$ and $y$ be $N \times 1$ discrete time signals.
	
	In DSP,
	\begin{align}\label{convform}
	x * y = \sum_{k = 0}^{N-1} y_{n-k}x_{k}
	\end{align}
	Equation \eqref{convform} can be written as the following matrix vector multiplication:
	\begin{align}
	x * y &= \begin{bmatrix}
	y_0  & y_{N-1} & y_{N-2} & \hdots & y_{2} & y_{1} \\
	y_{1}  & y_{0} & y_{N-1} &  \hdots & y_{3} & y_{2} \\
	y_{2}  & y_{1} & y_{0} &  \hdots & y_{4} & y_{3} \\
	\vdots  & \vdots & \vdots & \ddots & \vdots  & \vdots\\
	y_{N-2}  & y_{N-3} & y_{N-4} &  \hdots & y_{0} & y_{N-1} \\
	y_{N-1}  & y_{N-2} & y_{N-3} &  \hdots & y_{1} & y_{0} \\
	\end{bmatrix} x \label{expandmtx}\\
	&= (y_0I + y_1A + y_2A^2 + \hdots + y_{N-1}A^{N-1})x \nonumber\\
    &= \left(\sum_{i = 0}^{N-1} y_{i}A^{i}\right)x \nonumber\\
	&= P(A)x \nonumber
	\end{align}
	Thus,
	\begin{align} \label{Apolydsp}
	 P(A) = \sum_{i = 0}^{N-1} y_{i}A^{i}
	\end{align}
	
    The $N \times N$ unitary DFT is given by:
    \begin{align} \label{dftmatrix}
    \textrm{DFT} = \frac{1}{\sqrt{N}}\left(e^{-\frac{2\pi j}{N}pq}\right)_{p,q = 0,1,2,\hdots,N-1}
    \end{align} where $j = \sqrt{-1}$.

    The Fourier pair is:
    \begin{align}\label{dftfourierpair1}
	P(A) \ x \xrightarrow{\mathcal{F}} \sqrt{N} \ (\widehat{y} \odot \widehat{x})
	\end{align}

	From Equation \eqref{convtimeansgen} and Equation \eqref{dftfourierpair1}, substituting in the DFT for the GFT and $k = \sqrt{N}$ yields:
	\begin{align} \label{dftA}
	P(A) = \sqrt{N} \left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \textrm{DFT}\right)
	\end{align}
	
	\begin{theorem}
	In DSP, the two formulations for $P(A)$ from the DSP convolution definition in Equation \eqref{Apolydsp} and from the GSP theory in Equation \eqref{dftA} are equivalent.
	\end{theorem}
	$P(A) = \sqrt{N} \left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \textrm{DFT}\right) = \sum_{i = 0}^{N-1} y_{i}A^{i}$
	\begin{proof}
	It suffices to show that $\sqrt{N} \left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \textrm{DFT}\right)$ is equal to the matrix of y values in Equation \eqref{expandmtx}.
	
	Let $P = P(A)$. Let $P_i$ denote the $i$th column of $P(A)$.
	\begin{align} \label{pieq}
	P_i = \sqrt{N}\left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \textrm{DFT}_i\right)
	\end{align}
    where $\textrm{DFT}_i$ is the $i$th column of the DFT matrix.

    So,
    \begin{align} \label{dftkmatrix}
    \textrm{DFT}_i = \frac{1}{\sqrt{N}}\left(e^{-\frac{2\pi j}{N}pi}\right)_{p = 0,1,2,\hdots,N-1}
    \end{align}
    Substituting Equation \eqref{dftkmatrix} into Equation \eqref{pieq}  yields:
    \begin{align*}
	P_i &= \sqrt{N}\left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \textrm{DFT}_i\right)\\
	&= \sqrt{N}\left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \frac{1}{\sqrt{N}}\left(e^{-\frac{2\pi j}{N}pi}\right)_{p = 0,1,2,\hdots,N-1}\right) \\
	&= \textrm{DFT}^{-1} \ \left(\widehat{Y}_p e^{-\frac{2\pi j}{N}pi}\right)_{p = 0,1,2,\hdots,N-1}\\
	&= y_{n-i}
    \end{align*}
    The $i$th column of $P(A)$ is equal to $y_n$ shifted $i$ times. This is precisely the matrix in Equation \eqref{expandmtxfreq}.
    So, $\sqrt{N}\left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{y}) \ \textrm{DFT}\right)$ is equal to the matrix of y values in Equation \eqref{expandmtxfreq}.
    Thus, the two formulations are equivalent.
	\end{proof}
	
	\textit{Example:}
	Let $N = 4$. Let $\widehat{X} = [1,2,3,4]^T$, $\widehat{Y}=[-1,1,2,4]^T$, $\widehat{Y} = \textrm{DFT} \ y=\frac{1}{2}[6,-3+3j,-4,-3-3j]^T$
	
	$A$ is the 4-node ring graph adjacency matrix:
	\begin{equation*}
	A = \begin{bmatrix}
	0  & 0 & 0 & 1 \\
	1  & 0 & 0 & 0 \\
	0 &	 1 & 0 & 0 \\
	0 &	 0 & 1 & 0
	\end{bmatrix}
	\end{equation*}
	
	From Equation \eqref{Apolydsp}, we have
	\begin{align*}
	    P(A) &= -I + A + 2A^2 + 4A^3 \\
	   &=
	\begin{bmatrix}
	-1  & 4 & 2 & 1 \\
	1  & -1 & 4 & 2 \\
	2 &	 1 & -1 & 4 \\
	4 &	 2 & 1 & -1
	\end{bmatrix}
	\end{align*}
	
	From Equation \eqref{dftA} with $k = 2$, we have
	\begin{align*}
	   P(A) &= 2\left(\textrm{DFT}^{-1} \ \textrm{diag}(\widehat{Y}) \ \textrm{DFT}\right)\\
	   &= 2\left(\textrm{DFT}^{-1} \ \textrm{diag}(\frac{1}{2}[6,-3+3j,-4,-3-3j]) \ \textrm{DFT}\right)\\
	   &= \textrm{DFT}^{-1} \ \textrm{diag}([6,-3+3j,-4,-3-3j]) \ \textrm{DFT} \\
	&= \begin{bmatrix}
	-1  & 4 & 2 & 1 \\
	1  & -1 & 4 & 2 \\
	2 &	 1 & -1 & 4 \\
	4 &	 2 & 1 & -1
	\end{bmatrix}
	\end{align*}
	Both formulations yield the matrix of y values detailed in Equation \eqref{expandmtx}.
	
	Thus,
	$x*y = P(A)x = \begin{bmatrix}
	-1  & 4 & 2 & 1 \\
	1  & -1 & 4 & 2 \\
	2 &	 1 & -1 & 4 \\
	4 &	 2 & 1 & -1
	\end{bmatrix} x = \begin{bmatrix}
	-1  & 4 & 2 & 1 \\
	1  & -1 & 4 & 2 \\
	2 &	 1 & -1 & 4 \\
	4 &	 2 & 1 & -1
	\end{bmatrix} [1,2,3,4]^T = [17, 19, 17, 7]^T$
	
	\subsection{DSP Convolution in Frequency} \label{subsec:dspfreqconvolution}
	We consider the $N$ node ring graph with adjacency matrix $A$. Let $x$ and $y$ be $N \times 1$ discrete time signals. $\widehat{X} = \textrm{DFT}\ x$, $\widehat{Y} = \textrm{DFT}\ y$. From Theorem \ref{AMequal}, we know that the frequency shift, $M = A$.
	
	In DSP,
	\begin{align}\label{convformfreq}
	\widehat{X} * \widehat{Y} = \sum_{k = 0}^{N-1} {\widehat{Y}_{n-k}\widehat{X}_{k}}
	\end{align}
	Equation \eqref{convformfreq} can be written as the following matrix vector multiplication:
	\begin{align}
	\widehat{X} * \widehat{Y} &= \begin{bmatrix}
	\widehat{Y}_0  & \widehat{Y}_{N-1} & \widehat{Y}_{N-2} & \hdots & \widehat{Y}_{2} & \widehat{Y}_{1} \\
	\widehat{Y}_{1}  & \widehat{Y}_{0} & \widehat{Y}_{N-1} &  \hdots & \widehat{Y}_{3} & \widehat{Y}_{2} \\
	\widehat{Y}_{2}  & \widehat{Y}_{1} & \widehat{Y}_{0} &  \hdots & \widehat{Y}_{4} & \widehat{Y}_{3} \\
	\vdots  & \vdots & \vdots & \ddots & \vdots  & \vdots\\
	\widehat{Y}_{N-2}  & \widehat{Y}_{N-3} & \widehat{Y}_{N-4} &  \hdots & \widehat{Y}_{0} & \widehat{Y}_{N-1} \\
	\widehat{Y}_{N-1}  & \widehat{Y}_{N-2} & \widehat{Y}_{N-3} &  \hdots & \widehat{Y}_{1} & \widehat{Y}_{0} \\
	\end{bmatrix} \widehat{X} \label{expandmtxfreq}\\
	&= (\widehat{Y}_0I + \widehat{Y}_1M + \widehat{Y}_2M^2 + \hdots + \widehat{Y}_{N-1}M^{N-1})x \nonumber \\
    &= \left(\sum_{i = 0}^{N-1} \widehat{Y}_{i}M^{i}\right)x \nonumber\\
	&= P(M)x \nonumber
	\end{align}
	Thus,
	\begin{align} \label{Mpolydsp}
	 P(M) = \sum_{i = 0}^{N-1} \widehat{Y}_{i}M^{i}
	\end{align}
    The $N \times N$ unitary $\textrm{DFT}^{-1}$ is given by:
    \begin{align} \label{dftmatrixinv}
     \textrm{DFT}^{-1} = \frac{1}{\sqrt{N}}\left(e^{\frac{2\pi j}{N}pq}\right)_{p,q = 0,1,2,\hdots,N-1}
    \end{align} where $j = \sqrt{-1}$.
    The Fourier pair is:
    \begin{align}\label{dftfourierpair2}
	\sqrt{N} (\widehat{y} \odot \widehat{x}) \xrightarrow{\mathcal{F}} P(M) \ x
	\end{align}
	From Equation \eqref{convfreqansgen}, substituting in the DFT for the GFT yields:
	\begin{align} \label{dftM}
	P(M) = \sqrt{N}\left(\textrm{DFT}\ \textrm{diag}(y) \ \textrm{DFT}^{-1}\right)
	\end{align}
	
	\begin{theorem}
	In DSP, the two formulations for $P(M)$ from the DSP convolution definition in Equation \eqref{Mpolydsp} and from the GSP theory in Equation \eqref{dftM} are equivalent.
	
    $P(M) = \sqrt{N}\left(\textrm{DFT} \ \textrm{diag}(y) \ \textrm{DFT}^{-1}\right) = \sum_{i = 0}^{N-1} \widehat{Y}_{i}M^{i}$
	\end{theorem}
	
	\begin{proof}
	It suffices to show that $\sqrt{N}\left(\textrm{DFT}\ \textrm{diag}(y) \ \textrm{DFT}^{-1}\right)$ is equal to the matrix of $\widehat{Y}$ values in Equation \eqref{expandmtxfreq}.
	
	Let $P = P(M)$. Let $P_i$ denote the $i$th column of $P(M)$.
	\begin{align} \label{pieqfreq}
	P_i = \sqrt{N}\left(\textrm{DFT} \ \textrm{diag}(y) \ \textrm{DFT}^{-1}_i\right)
	\end{align}
    where $\textrm{DFT}^{-1}_i$ is the $i$th column of the $\textrm{DFT}^{-1}$ matrix.



    So,
    \begin{align} \label{dftkmatrixinv}
    \textrm{DFT}_i = \frac{1}{\sqrt{N}}\left(e^{\frac{2\pi j}{N}pi}\right)_{p = 0,1,2,\hdots,N-1}
    \end{align}
    Substituting Equation \eqref{dftkmatrixinv} into Equation \eqref{pieqfreq}  yields:
    \begin{align*}
	P_i &= \sqrt{N}\left(\textrm{DFT} \ \textrm{diag}(y) \ \textrm{DFT}^{-1}_i\right)\\
	&= \sqrt{N}\left(\textrm{DFT} \ \textrm{diag}(y) \ \frac{1}{\sqrt{N}}\left(e^{\frac{2\pi j}{N}pi}\right)_{p = 0,1,2,\hdots,N-1}\right) \\
	&= \textrm{DFT} \ \left(y_p e^{-\frac{2\pi j}{N}pi}\right)_{p = 0,1,2,\hdots,N-1} \\
	&= \widehat{Y}_{n-i}
    \end{align*}
    The $i$th column of $P(M)$ is equal to $\widehat{Y}_{n}$ shifted i times. This is precisely the matrix in Equation \eqref{expandmtxfreq}.
    So, $\sqrt{N}\left(\textrm{DFT} \ \textrm{diag}(y) \ \textrm{DFT}^{-1}\right)$ is equal to the matrix of $\widehat{Y}$ values in Equation \eqref{expandmtxfreq}.
    Thus, the two formulations are equivalent.
	\end{proof}
	
	\textit{Example:}
	Let $N = 4$. Let $\widehat{X} = [1,2,3,4]^T$, $\widehat{Y}=[6,-3+3j,-4,-3-3j]^T$, $y = \textrm{DFT}^{-1} \ \widehat{Y}=\frac{1}{2}[-4, 16, 8, 4]^T$
	
	$A$ is the 4-node ring graph adjacency matrix. Using Theorem \ref{AMequal},
	\begin{equation*}
	M = A = \begin{bmatrix}
	0  & 0 & 0 & 1 \\
	1  & 0 & 0 & 0 \\
	0 &	 1 & 0 & 0 \\
	0 &	 0 & 1 & 0
	\end{bmatrix}
	\end{equation*}
	
	From Equation \eqref{Mpolydsp}, we have
	\begin{align*}
	    P(M) &= 6I + (-3+3j)A + -4A^2 + (-3-3j)A^3 \\
	   &=
	\begin{bmatrix}
	6  & -3+3j & -4 & -3-3j \\
	-3-3j  & 6 & -3+3j & -4 \\
	-4 & -3-3j & 6 & -3+3j \\
	-3+3j &	 -4 & -3-3j & 6
	\end{bmatrix}
	\end{align*}
	
	From Equation \eqref{dftM}, we have
	\begin{align*}
	   P(M) &= 2\left(\textrm{DFT} \ \textrm{diag}(y) \ \textrm{DFT}^{-1}\right)\\
	   &= 2\left(\textrm{DFT} \ \textrm{diag}(\frac{1}{2}[-4, 16, 8, 4]) \ \textrm{DFT}^{-1}\right)\\
	   &= \textrm{DFT} \ \textrm{diag}([-4,16,8,4]) \ \textrm{DFT}^{-1}\\
	&= \begin{bmatrix}
	6  & -3+3j & -4 & -3-3j \\
	-3-3j  & 6 & -3+3j & -4 \\
	-4 & -3-3j & 6 & -3+3j \\
	-3+3j &	 -4 & -3-3j & 6
	\end{bmatrix}
	\end{align*}
	Both formulations yield the matrix of y values detailed in Equation \eqref{expandmtxfreq}.
	
	Thus,
	$\widehat{x}*\widehat{y} = P(M)x = \\
	\begin{bmatrix}
	6  & -3+3j & -4 & -3-3j \\
	-3-3j  & 6 & -3+3j & -4 \\
	-4 & -3-3j & 6 & -3+3j \\
	-3+3j &	 -4 & -3-3j & 6
	\end{bmatrix} \widehat{x} =  \\ \begin{bmatrix}
	6  & -3+3j & -4 & -3-3j \\
	-3-3j  & 6 & -3+3j & -4 \\
	-4 & -3-3j & 6 & -3+3j \\
	-3+3j &	 -4 & -3-3j & 6
	\end{bmatrix} [1,2,3,4]^T \\ = [-24-6j, -16+6j, -4+6j, 4-6j]^T$



	
	\subsection{Polynomials of the Shift}
	In the previous two sections, we illustrated two ways
	
	
	
	
	
	
	
	\subsection{Scaling Constants}
	The eigendecomposition of $A$ is subject to scaling constants. The GFT matrix can be scaled by a factor of $k$ and the $\textrm{GFT}^{-1}$ can be scaled by a factor of $\frac{1}{k}$.
	For example, suppose $A$ has eigendecomposition, $A = \textrm{GFT}^{-1} \ \Lambda \ \textrm{GFT}$. Then,
	\begin{equation} \label{alteigen}
	A = k \ \textrm{GFT}^{-1} \ \Lambda \ \textrm{GFT} \ \frac{1}{k}
	\end{equation}
	where $k \in \mathbb{R}$, $k \neq 0$ is also a valid eigendecomposition of $A$. However, the GFT and $\textrm{GFT}^{-1}$ have been scaled by constants, producing different numerical results and Fourier pairs. Because of this, we now introduce a generic form of Equation \eqref{convpairtime}:
	\begin{equation}\label{convpairtimegen}
	P(A) \ x \xrightarrow{\mathcal{F}} k\ \left(\widehat{y} \odot \widehat{x}\right)
	\end{equation}
	where $x$ and $y$ are signals, $k \in \mathbb{R}$ is a scalar, and $P(A)$ is the polynomial of $A$.
	Based on Equation \eqref{convpairtimegen}, using a similar argument as in Section A, we can derive the following generic form of Equation \eqref{convtimeans}.
	\begin{align}
	    P(\Lambda)\widehat{x} &= k\left(\widehat{y}\odot\widehat{x}\right) \nonumber\\
	    P(\Lambda) &= k\left(\textrm{diag}(\widehat{y})\right) \nonumber\\
	    P(A) &= k \left( \textrm{GFT}^{-1} \ \textrm{diag}(\widehat{y}) \ \textrm{GFT}\right)  \label{convtimeansgen}
	\end{align}
	
	Similarly, for convolution in the spectral domain, we introduce a generic form of Equation \eqref{convpair}:
	\begin{equation}\label{convpairgen}
	l\left(y \odot x\right) \xrightarrow{\mathcal{F}} P(M) \ \widehat{x}
	\end{equation}
	where $x$ and $y$ are signals, $l\in \mathbb{R}$ is a scalar and $P(M)$ is a polynomial of the graph shift in frequency, $M$. Based on Equation \eqref{convpairgen}, using a similar argument as in Section B, we can derive a generic form of Equation \eqref{convfreqans}.
	\begin{align}
	    P(\Lambda^*)x &= l\left(y \odot x\right) \nonumber\\
	    P(\Lambda^*) &= l\left(\textrm{diag}(y)\right) \nonumber\\
	    P(M) &= l \left( \textrm{GFT} \ \textrm{diag}(y) \ \textrm{GFT}^{-1}\right)  \label{convfreqansgen}
	\end{align}

	This theory is also consistent with DSP by considering matrix $M$ in equation \eqref{Meqn} and the adjacency matrix $A$ of the $N$ node ring graph. We will illustrate this theoretically and by example in the next sections.

